Traffic Flow Optimisation for Lifelong Multi-Agent Path Finding

Multi-Agent Path Finding (MAPF) is a fundamental problem in robotics that asks us to compute collision-free paths for a team of agents, all moving across a shared map. Although many works appear on this topic, all current algorithms struggle as the number of agents grows. The principal reason is that existing approaches typically plan free-flow optimal paths, which creates congestion. To tackle this issue, we propose a new approach for MAPF where agents are guided to their destination by following congestion-avoiding paths. We evaluate the idea in two large-scale settings: one-shot MAPF, where each agent has a single destination, and lifelong MAPF, where agents are continuously assigned new destinations. Empirically, we report large improvements in solution quality for one-short MAPF and in overall throughput for lifelong MAPF.

==> algs/enum.tex <==
% algorithmic commands

\ignore{
\newcommand{\Break}{\textbf{break}}
\algnewcommand{\IfThen}[2]{% \IfThenElse{<if>}{<then>}{<else>}
  \State \algorithmicif\ #1\ \algorithmicthen\ #2}
\algnewcommand{\IfThenElse}[3]{% \IfThenElse{<if>}{<then>}{<else>}
  \State \algorithmicif\ #1\ \algorithmicthen\ #2\ \algorithmicelse\ #3}
\begin{algorithm}[t]
  \begin{algorithmic}[1]
    \Procedure{XpEnum}{$\kappa$, $\mbf{v}$, $c$}
      \State $\left(\axps, \cxps\right)\gets (\emptyset, \emptyset)$ \label{ln:init}
      \Comment{Sets of AXp's and CXp's to collect.}
      \While{true}
        \State $\fml{Y}\gets\Call{MinimalHS}{\axps, \cxps}$ \label{ln:mhs}
        \Comment{Get a new MHS of $\axps$ subject to $\cxps$.}
        \IfThen{$\fml{Y}=\bot$}{\Break} \label{ln:nocand}
        \Comment{Stop if none is computed.}
        % \If{$\Call{IsCXp}{\fml{Y},\kappa,\mbf{v},c}$}
        \If{$\exists(\mbf{x}\in\mbb{F}).\bigwedge\nolimits_{i\not\in\fml{Y}}(x_i=v_i)\land(\kappa(\mbf{x})\not=c)$} \label{ln:check}
          \Comment{Check CXp condition \eqref{eq:cxp} for $\fml{Y}$.}
          \State $\cxps\gets\cxps\cup\{\fml{Y}\}$ \label{ln:cxprec}
          \Comment{$\fml{Y}$ appears to be a CXp.}
        \Else
          \Comment{There must be a missing AXp $\fml{X}\subseteq\fml{F}\setminus\fml{Y}$.}
          \State $\fml{X}\gets\Call{ExtractAXp}{\fml{F}\setminus\fml{Y},\kappa,\mbf{v},c}$ \label{ln:extract}
          \Comment{Get AXp $\fml{X}$ by iteratively checking~\eqref{eq:axp}~\cite{inms-aaai19}.}
          \State $\axps\gets\axps\cup\{\fml{X}\}$ \label{ln:axprec}
          \Comment{Collect new AXp $\fml{X}$.}
        \EndIf
      \EndWhile
      \Return{$\axps$, $\cxps$}
    \EndProcedure
  \end{algorithmic}
  \caption{MARCO-like Anytime Explanation Enumeration}
  \label{alg:enum}
\end{algorithm}
}

\begin{algorithm}[t]
	\caption{MARCO-like Anytime Explanation Enumeration}\label{alg:enum}
	%\textbf{Input}: Dataset $\fml{E}$, extraction limit  $\lambda$ \\
	\textbf{Input}: Classifier~$\kappa$, instance~$\mbf{v}$, prediction~$c=\kappa(\mbf{v})$  \\ 
	%\textbf{Output}: Rules $\varphi$
	\textbf{Output}: AXp’s~$\axps$, CXp’s~$\cxps$
	\begin{algorithmic}[1]
		\STATE $\left(\axps, \cxps\right)\gets (\emptyset, \emptyset)$ \label{ln:init}
	        \COMMENT{Sets of AXp's and CXp's to collect.}
		\WHILE{true}
			\State $\fml{Y}\gets\Call{MinimalHS}{\axps, \cxps}$ \label{ln:mhs}
			\COMMENT{Get a new MHS of $\axps$ subject to $\cxps$.}
		\ENDWHILE
		%\FOR {$i \in \fml{F}$} \label{line:forfeat}
		%\FOR {$\textsf{rule}\in \texttt{EnumerateRules}(\fml{E}_f, i, B$)}
		%\IF {\texttt{limit}($\textsf{rule}, \lambda$) is $true$}
		%\STATE \textbf{break}
		%\ENDIF
		%\STATE $\varphi \gets  \varphi \cup \textsf{rule}$
		%\ENDFOR
		%\STATE $B \gets \varphi$
		%\ENDFOR
		%\RETURN $\varphi$
	\end{algorithmic}
\end{algorithm}

\ignore{
\begin{algorithm}[t]
	\caption{Rule Extraction}\label{alg:rextract}
	\textbf{Input}: Dataset $\fml{E}$, extraction limit  $\lambda$ \\
	\textbf{Output}: Rules $\varphi$
	\begin{algorithmic}[1]
		\STATE $\fml{E}_f, \fml{F} \gets \texttt{DropClass}(\fml{E}), \texttt{ExtractFeatures}(\fml{E})$
		\STATE $\varphi, B \gets \emptyset, \emptyset $ \COMMENT{to extract and block rules, resp.}
		\FOR {$i \in \fml{F}$} \label{line:forfeat}
		\FOR {$\textsf{rule}\in \texttt{EnumerateRules}(\fml{E}_f, i, B$)}
		\IF {\texttt{limit}($\textsf{rule}, \lambda$) is $true$}
		\STATE \textbf{break}
		\ENDIF
		\STATE $\varphi \gets  \varphi \cup \textsf{rule}$
		\ENDFOR
		\STATE $B \gets \varphi$
		\ENDFOR
		\RETURN $\varphi$
	\end{algorithmic}
\end{algorithm}
}


==> relw.tex <==
q\section{Related Work} \label{sec:relw}


==> texfigs/bt.tex <==
%------------------------------------------------------------------------------%
% File:        bt.tex
%
% Description:
%
% Created:     7 Feb 2018.
%
% Author:      Alexey Ignatiev (aign).
%------------------------------------------------------------------------------%

% defining box structure
\tikzstyle{box} = [draw=black!90, thick, rectangle, rounded corners,
                     inner sep=10pt, inner ysep=20pt, dotted
                  ]
\tikzstyle{title} = [draw=black!90, fill=black!5, semithick, top color=white,
                     bottom color = black!5, text=black!90, rectangle,
                     font=\small, inner sep=2pt, minimum height=1.3em,
                     top color=tyellow2!27, bottom color=tyellow2!27
                    ]
% block styles
\tikzstyle{feature} = [rectangle,font=\scriptsize,rounded corners=1mm,thick,%
                       draw=black!80, top color=tblue2!20,bottom color=tblue2!25,%
                       draw, minimum height=1.1em, text centered,%
                       inner sep=2pt%
                      ]
\tikzstyle{pscore} = [rectangle,font=\scriptsize,rounded corners=1mm,thick,%
                     draw=black!80, top color=tgreen3!20,bottom color=tgreen3!27,%
                     draw, minimum height=1.1em, text centered,%
                     inner sep=2pt%
                    ]
\tikzstyle{nscore} = [rectangle,font=\scriptsize,rounded corners=1mm,thick,%
                     draw=black!80, top color=tred2!20,bottom color=tred2!25,%
                     draw, minimum height=1.1em, text centered,%
                     inner sep=2pt%
                    ]

\begin{adjustbox}{center}
\setlength{\tabcolsep}{3pt}
\def\arraystretch{3}
\begin{tabular}{ccc}
    \begin{tikzpicture}[node distance = 4.0em, auto]
        % creating a box with the title
        \node [box] (box) {%
        \begin{minipage}[t!]{0.314\textwidth}
            \vspace{0.9cm}\hspace{1.5cm}
        \end{minipage}
        };
        \node[title] at (box.north) {$\text{T}_\text{1}$ ($\geq 50$k)};

        % feature node
        \node [feature] (feat1) at (0.016, 0.57) {Status $=$ Married?};
        \node [feature, below left  = 0.8em and -2.78em of feat1] (feat2) {Education $=$ Dropout?};
        \node [feature, below right = 0.8em and -2.78em of feat1] (feat3) {Rel. $=$ Not-in-family?};

        % leaf nodes
        \node [nscore, below left  = 0.8em and -2.8em of feat2] (pos1) {-0.1569};
        \node [pscore, below right  = 0.8em and -2.8em of feat2] (neg1) {0.0770};
        \node [nscore, below left = 0.8em and -2.8em of feat3] (pos2) {-0.1089};
        \node [nscore, below right = 0.8em and -2.8em of feat3] (neg2) {-0.3167};

        % arrows to the leaves
        \draw [->,thick,black!80] (feat1) to[] node[above, pos=1.2, font=\scriptsize] {yes} (feat2.north);
        \draw [->,thick,black!80] (feat1) to[] node[above, pos=1.1, font=\scriptsize] { no} (feat3.north);
        \draw [->,thick,black!80] (feat2) to[] node[above, pos=1.2, font=\scriptsize] {yes} (pos1.north);
        \draw [->,thick,black!80] (feat2) to[] node[above, pos=1.1, font=\scriptsize] { no} (neg1.north);
        \draw [->,thick,black!80] (feat3) to[] node[above, pos=1.2, font=\scriptsize] {yes} (pos2.north);
        \draw [->,thick,black!80] (feat3) to[] node[above, pos=1.1, font=\scriptsize] { no} (neg2.north);
    \end{tikzpicture}
    &
    \begin{tikzpicture}[node distance = 4.0em, auto]
        % creating a box with the title
        \node [box] (box) {%
        \begin{minipage}[t!]{0.302\textwidth}
            \vspace{0.9cm}\hspace{1.5cm}
        \end{minipage}
        };
        \node[title] at (box.north) {$\text{T}_\text{2}$ ($\geq 50$k)};

        % feature node
        \node [feature] (feat1) at (-0.335, 0.57) {Hours/w $\leq$ 40?};
        \node [feature, below left  = 0.8em and -2.36em of feat1] (feat2) {Status $=$ Married?};
        \node [feature, below right = 0.8em and -2.36em of feat1] (feat3) {Status $=$ Never-Married?};

        % leaf nodes
        \node [nscore, below left  = 0.8em and -2.8em of feat2] (pos1) {-0.0200};
        \node [nscore, below right  = 0.8em and -2.8em of feat2] (neg1) {-0.2404};
        \node [nscore, below left = 0.8em and -2.8em of feat3] (pos2) {-0.1245};
        \node [pscore, below right = 0.8em and -2.8em of feat3] (neg2) {0.0486};

        % arrows to the leaves
        \draw [->,thick,black!80] (feat1) to[] node[above, pos=1.2, font=\scriptsize] {yes} (feat2.north);
        \draw [->,thick,black!80] (feat1) to[] node[above, pos=1.1, font=\scriptsize] { no} (feat3.north);
        \draw [->,thick,black!80] (feat2) to[] node[above, pos=1.2, font=\scriptsize] {yes} (pos1.north);
        \draw [->,thick,black!80] (feat2) to[] node[above, pos=1.1, font=\scriptsize] { no} (neg1.north);
        \draw [->,thick,black!80] (feat3) to[] node[above, pos=1.2, font=\scriptsize] {yes} (pos2.north);
        \draw [->,thick,black!80] (feat3) to[] node[above, pos=1.1, font=\scriptsize] { no} (neg2.north);
    \end{tikzpicture}
    &
     \begin{tikzpicture}[node distance = 4.0em, auto]
        % creating a box with the title
        \node [box] (box) {%
        \begin{minipage}[t!]{0.28\textwidth}
            \vspace{0.9cm}\hspace{1.5cm}
        \end{minipage}
        };
        \node[title] at (box.north) {$\text{T}_\text{3}$ ($\geq 50$k)};

        % feature node
        \node [feature] (feat1) at (0.113, 0.57) {Education $=$ Doctorate?};
        \node [feature, below left  = 0.8em and -3.6em of feat1] (feat2) {40 $<$ Hours/w $\leq$ 45?};
        \node [feature, below right = 0.8em and -3.6em of feat1] (feat3) {Rel. $=$ Own-child?};

        % leaf nodes
        \node [pscore, below left  = 0.8em and -2.8em of feat2] (pos1) {0.0605};
        \node [pscore, below right  = 0.8em and -2.8em of feat2] (neg1) {0.3890};
        \node [nscore, below left = 0.8em and -2.8em of feat3] (pos2) {-0.2892};
        \node [nscore, below right = 0.8em and -2.8em of feat3] (neg2){-0.0580};

        % arrows to the leaves
        \draw [->,thick,black!80] (feat1) to[] node[above, pos=1.2, font=\scriptsize] {yes} (feat2.north);
        \draw [->,thick,black!80] (feat1) to[] node[above, pos=1.1, font=\scriptsize] { no} (feat3.north);
        \draw [->,thick,black!80] (feat2) to[] node[above, pos=1.2, font=\scriptsize] {yes} (pos1.north);
        \draw [->,thick,black!80] (feat2) to[] node[above, pos=1.1, font=\scriptsize] { no} (neg1.north);
        \draw [->,thick,black!80] (feat3) to[] node[above, pos=1.2, font=\scriptsize] {yes} (pos2.north);
        \draw [->,thick,black!80] (feat3) to[] node[above, pos=1.1, font=\scriptsize] { no} (neg2.north);
    \end{tikzpicture}
    \\
   \end{tabular}
\end{adjustbox}

%------------------------------------------------------------------------------%


